Unsupervised Multi-document Summarization with Holistic Inference

Multi-document summarization aims to obtain core information from a collection of documents written on the same topic. This paper proposes a new holistic framework for unsupervised multi-document extractive summarization. Our method incorporates the holistic beam search inference method associated with the holistic measurements, named Subset Representative Index (SRI). SRI balances the importance and diversity of a subset of sentences from the source documents and can be calculated in unsupervised and adaptive manners. To demonstrate the effectiveness of our method, we conduct extensive experiments on both small and large-scale multi-document summarization datasets under both unsupervised and adaptive settings. The proposed method outperforms strong baselines by a significant margin, as indicated by the resulting ROUGE scores and diversity measures. Our findings also suggest that diversity is essential for improving multi-document summary performance.

==> tables/alg_exh.tex <==
\begin{algorithm}[tb]
\small
\caption{Exhaustive Set}
\label{alg:exhaustive}
\textbf{Input}: Set of sentences $\mathcal{S}$, Measurement $\mathcal{M}(\cdot)$  \\
\textbf{Parameter}: Num. of summary Sent. $N < |\mathcal{S}|$\\
\textbf{Output}: Selected Subset $\mathcal{S'}$
\begin{algorithmic}[1] %[1] enables line numbers
\STATE Let $\mathcal{S'}=\varnothing$.
\FOR{$\mathcal{X} \subset \mathcal{S}$ and $|\mathcal{X}| = N$}
\IF{$\mathcal{M}(\mathcal{X}) > \mathcal{M}(\mathcal{S'})$}
    \STATE $\mathcal{S'} \gets \mathcal{X}$
\ENDIF
\ENDFOR
\STATE \textbf{return} $\mathcal{S'}$
\end{algorithmic}
\end{algorithm}

==> tables/alg_greedy.tex <==
\begin{algorithm}[tb]
\small
\caption{Greedy Set}
\label{alg:greedy}
\textbf{Input}: Set of sentences $\mathcal{S}$, Measurement $\mathcal{M}(\cdot)$  \\
\textbf{Parameter}: Num. of summary Sent. $N < |\mathcal{S}|$\\
\textbf{Output}: Selected Subset $\mathcal{S'}$
\begin{algorithmic}[1] %[1] enables line numbers
\STATE Let $\mathcal{S'}=\varnothing$.
\WHILE{$|\mathcal{S'}| < N$}
\STATE $x \gets \argmax_{s_i \in \mathcal{S} \setminus \mathcal{S'}} \mathcal{M}(\mathcal{S'} \cup \{s_i\})$ 
\STATE $\mathcal{S'} \gets \mathcal{S'} \cup \{x\} $
\ENDWHILE
\STATE \textbf{return} $\mathcal{S'}$
\end{algorithmic}
\end{algorithm}

==> tables/algorithm.tex <==
\begin{algorithm}[tb]
\caption{Decoding with DPP}
\label{alg:algorithm}
\textbf{Input}: Document Cluster $\mathcal{C}$, ensemble matrix $L$, summary length $k$\\
% \textbf{Parameter}: Optional list of parameters\\
\textbf{Output}: Summary $S$\\
\hrule
\textbf{Greedy Sentence Decoding}
\begin{algorithmic} [1]%[1] enables line numbers
\STATE $S = \emptyset$
\WHILE{$|S|<k$}
\STATE extract sentence $s_i$ by $\argmax{P}(s;L)$
\STATE $S = S\cup s_i$
\STATE $L = L-L_{s_i}$
\STATE back to 2
\ENDWHILE
\STATE \textbf{return} summary S
\end{algorithmic}   
\hrule
\textbf{Greedy Set Decoding}
\begin{algorithmic}[1]
\STATE $S = \emptyset$
\WHILE{$|S|<k$}
\STATE extract sentence $s_i$ by $\argmax_{s_j \in \mathcal{C}}{P}(S\cup s_i;L) $
\STATE $S = S\cup s_i$
\STATE back to 2
\ENDWHILE
\STATE \textbf{return} summary S
\end{algorithmic}
\hrule
\textbf{Subgraph Decoding}
\begin{algorithmic}[1]

\STATE candidate pruning to $p$ based on centrality ranking
\STATE generate ${p \choose k}$ candidate subgraphs $\mathcal{S}$
\STATE $summary= \arg\max_{S \in \mathcal{S}} \mathbf{P}(S;L))$

\STATE back to 2

\STATE \textbf{return} summary S
\end{algorithmic}
\end{algorithm}

==> tables/result_duc.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.25}
\centering
\begin{small}
\scalebox{1}{
\begin{tabular}{|l|ccc|ccc|}
\hline
& \multicolumn{3}{c|}{\textbf{\textsl{DUC-04}}} & \multicolumn{3}{c|}{\textbf{\textsl{TAC-11}}}\\
\textbf{System} & \textbf{R-1} & \textbf{R-2} & \textbf{R-SU}  & \textbf{R-1} & \textbf{R-2} & \textbf{R-SU}  \\
\hline
% \rowcolor{gray!10}
% \multicolumn{7}{|c|}{\textbf{\textsl{Supervised Systems}}} \\
% \hline
% Opinosis (\citeyear{Ganesan:2010}) &27.07& 5.03&8.63&25.15& 5.12&8.12\\
% Extract+RW (\citeyear{song2018structure}) &28.90&5.33&8.76&29.07&6.11&9.20\\
% Pointer-Gen (\citeyear{see2017get}) &31.43&6.03&10.01&31.44&6.40&10.20\\
% PG-MMR (\citeyear{lebanoff-etal-2018-adapting}) &{36.88} &{8.73}  &{12.64}&{37.17}&{10.92}&{14.04}\\
% DPP-BERT (\citeyear{cho2019multi}) &\textbf{39.05} &\textbf{10.23}  &\textbf{14.35}&\textbf{38.59}&\textbf{ 11.06}&\textbf{14.65}\\
% \hline
\rowcolor{gray!10}
\multicolumn{7}{|c|}{\textbf{\textsl{Unsupervised Systems}}} \\
\hline
% \textsc{Oracle} & 55.40 & 29.91 & 50.51 & &  & 49.43 & 27.18 & 45.04 & & \\
LEAD &30.77&8.27&7.35& 32.88&7.84&11.46\\

MMR (\citeyear{carbonell1998use}) &30.14&4.55&8.16&-&-&-\\
LexRank (\citeyear{Erkan:2004})& 34.44 & 7.11 & 11.19  & 33.10 & 7.50 & 11.13 \\

SumBasic (\citeyear{vanderwende2007beyond})&   29.48 & 4.25 & 8.64  & 31.58 & 6.06 & 10.06 \\
KLSumm (\citeyear{haghighi2009exploring})&31.04&6.03&10.23&31.23&7.07&10.56\\
\hline
\rowcolor{gray!10}
\multicolumn{7}{|c|}{\textbf{\textsl{Our Methods}}} \\
\hline
Sent. + greedy &34.81&7.85&11.37&34.42&8.10&11.25\\
% SRI + greedy sent. &\textbf{36.59}&\textbf{8.39}&\textbf{12.33}&\textbf{35.06}&\textbf{8.28}&\textbf{12.14}\\
SRI + beam &\textbf{36.84}&\textbf{8.37}&{12.28}&{35.37}&\textbf{8.49}&\textbf{11.73}\\
SRI + exh w/ filter &{36.70}&\textbf{8.37}&\textbf{12.31}&{35.19}&{8.31}&{11.34}\\
% DPP + greedy sent. &34.82&7.85&11.41&34.42&8.10&11.62\\
% DPP + beam &35.71&6.79&10.94&34.06&6.66&10.68\\
% DPP + exh w/ filter &36.71&7.06&11.32&\textbf{36.08}&7.06&11.09\\
% Centrality&  {35.00} & {7.68} & {29.70} &     {36.19} & {9.43} &{31.27}   \\ 
% Cen.+MMR&  {37.15} & {8.75} & {32.15} &     {36.91} & {9.64} &{32.23}   \\ 
% Subgraph Cen.&  {36.17} & {8.45} & {30.39} &     {36.31} & {9.32} &{30.98}   \\ 
% Cen.+DPP&  {36.84} & {8.86} & {32.70} &     {37.45} & {9.82} &{32.35}   \\ 
\hline
\end{tabular}}
\end{small}
\caption{ROUGE-F1 results on DUC-04 and TAC-11 datasets. Best supervised and unsupervised results are bold.
For fair comparison, the ROUGE scores are calculated with 100 words limit.
%\textcolor{red}{TO DO: generate results on LEAD or we remove the LEAD baseline in \Cref{tab:results_duc}}
}
\label{tab:results_duc}
\end{table}

==> tables/result_news.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.25}
\centering
\begin{small}\scalebox{0.9}{
\begin{tabular}{|l|ccc|ccc|}
\hline
& \multicolumn{3}{c|}{\textbf{\textsl{MultiNews}}} & \multicolumn{3}{c|}{\textbf{\textsl{WikiSum}}}\\
\textbf{System} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L*} \\
\hline
% \textsc{Oracle} & 55.40 & 29.91 & 50.51 & 49.43 & 27.18 & 45.04 \\
% \hline
% \rowcolor{gray!10}
% \multicolumn{7}{|c|}{\textbf{\textsl{remove- Supervised Systems}}} \\
% \hline
% P-Gen \citeyearpar{see2017get}&42.80&14.19&16.75&-&-&-\\
% FT~\citeyearpar{liu-lapata-2019-hierarchical}&44.32&15.11&20.50&40.56&25.35&34.73\\
% HT~\citeyearpar{liu-lapata-2019-hierarchical} & 42.36 & 15.27 & 22.08 & 41.53 & 26.52 & 35.76 \\
% PRIMERA~\citeyearpar{xiao-etal-2022-primera} &\textbf{49.90}&\textbf{21.10}&\textbf{25.90}&-&-&- \\

\rowcolor{gray!10}
\multicolumn{7}{|c|}{\textbf{\textsl{Unsupervised Systems}}} \\
\hline
\textsc{Lead} &   39.41 & 11.77 & 14.51 & 37.63 & 14.75 & 34.76 \\
MMR~\citeyearpar{carbonell1998use}&             38.77 & 11.98 & 12.91 & 31.22 & 10.24 & 22.48 \\
LexRank~\citeyearpar{Erkan:2004} &         38.27 & 12.70 & 13.20 & 36.12 & 11.67 & 22.52 \\
TextRank~\citeyearpar{mihalcea2004textrank}&        38.44 & 13.10 & 13.50 & 23.66 & 7.79 &  21.23 \\
DASG~\citeyearpar{liu2021unsupervised} &{42.60 }&{13.22}&{16.15}&-&-&- \\
% FAR~\citeyearpar{liang2021improving} &{43.48}&{16.87}&{ 44.00}&38.11&14.54&35.01 \\
PRIMERA~\citeyearpar{xiao-etal-2022-primera}&         42.00 & 13.60 & 20.80 & 28.00 & 8.00 & 18.00 \\
\hline
% Centrality &      40.48 & 13.49 & 36.81 & 35.85 & 11.94 & 32.64 \\
% cen.+MMR&43.64&14.05&39.46&&&\\
% Subgraph cen.&43.24&\textbf{14.62}&39.21&&&\\
% Cen.+DPP &        \textbf{44.13} & {14.00} & \textbf{40.24} & \textbf{39.02} & \textbf{16.02} & \textbf{34.64}  \\ 
\rowcolor{gray!10}
\multicolumn{7}{|c|}{\textbf{\textsl{Our Methods}}} \\
\hline
% SRI + greedy sent. & 404823389 &7.85 & 36.46 & 38.43& 10.74 & 33.18 \\
Sent. Greedy&40.48&13.49&16.14&37.24&10.29&32.77\\
SRI + beam & \textbf{44.22} & \textbf{14.63} & 18.61 & 38.94& 15.23 & 34.12 \\
SRI + exh & 43.16 &  {14.58} & {18.00} &\textbf{39.26} & \textbf{16.15} & {34.19} \\
% DPP + greedy sent. & {40.48} & {13.49} & {36.81} & {37.24} & {10.29} & {32.95}  \\ 
% DPP + beam & {44.12} & {14.43} & {17.83} & {38.42} & {13.46} & {32.85}  \\ 
% DPP + exh.w/filter & {44.13} & {14.00} & \textbf{18.63} & {39.02} & {16.02} & \textbf{34.64}  \\
\hline
\end{tabular}} 
\end{small}
\caption{ROUGE-F1 scores on the MultiNews and WikiSum datasets. Best supervised and unsupervised results are bold. For a fair comparison, we report {R-L} on Multinews and {R-Lsum}~\cite{see2017get} for WikiSum. \textcolor{blue}{remove caption}
}
\label{tab:results_news}
\end{table}
